Convex and Nonconvex Optimization Are Both Minimax-Optimal for Noisy Blind Deconvolution under Random Designs

We investigate the effectiveness of convex relaxation and nonconvex optimization in solving bilinear systems of equations under two different designs (i.e.$~$a sort of random Fourier design and Gaussian design). Despite the wide applicability, the theoretical understanding about these two paradigms remains largely inadequate in the presence of random noise. The current paper makes two contributions by demonstrating that: (1) a two-stage nonconvex algorithm attains minimax-optimal accuracy within a logarithmic number of iterations. (2) convex relaxation also achieves minimax-optimal statistical accuracy vis-\`a-vis random noise. Both results significantly improve upon the state-of-the-art theoretical guarantees.

==> proof_outline.tex <==

\section{Proof outline for Theorem \ref{theorem:cvx}\label{sec:Proof-outline-for-theorem-cvx}}

Since the proof of Theorem \ref{theorem:cvx} is more complicated
than that of Theorem \ref{theorem:gaussian-cvx} and they fall into
the same framework, we only sketch the proof of Theorem \ref{theorem:cvx}
here. As the empirical evidence (cf.~Figure \ref{fig:dist_cvx_ncvx})
suggests, an approximate nonconvex optimizer produced by a simple
gradient-type algorithm is exceedingly close to the convex minimizer
of (\ref{eq:objcvx}). In what follows, we shall start by introducing
an auxiliary nonconvex gradient method, and formalize its connection
to the convex program. Without loss of generality, we assume that $\Vert\bm{h}^{\star}\Vert_{2}=\Vert\bm{x}^{\star}\Vert_{2}=1$ throughout the proof. 

\paragraph{An auxiliary nonconvex algorithm.} Let us consider the
iterates obtained by running a variant of (Wirtinger) gradient descent,
as summarized in Algorithm \ref{alg:gd-bd-ncvx-2}. A crucial difference
from Algorithm \ref{alg:gd-BD-ncvx} lies in the initialization stage
--- namely, Algorithm \ref{alg:gd-bd-ncvx-2} initializes the algorithm
from the ground truth $(\bm{h}^{\star},\bm{x}^{\star})$ rather than
a spectral estimate as adopted in Algorithm \ref{alg:gd-BD-ncvx}.
While initialization at the truth is not practically implementable,
it is introduced here solely for analytical purpose, namely, it creates a sequence of ancillary random variables that approximate our estimators and are close to the ground truth. This is how we establish the convergence rate of our estimators.

\begin{algorithm}[h]
\caption{Auxiliary gradient descent for blind deconvolution (for analysis purpose only)}

\label{alg:gd-bd-ncvx-2}\begin{algorithmic}

\STATE \textbf{{Input}}: $\left\{ \bm{a}_{j}\right\} _{1\leq j\leq m}$,
$\left\{ \bm{b}_{j}\right\} _{1\leq j\leq m}$, $\left\{ y_{j}\right\} _{1\leq j\leq m}$,
$\bm{h}^{\star}$ and $\bm{x}^{\star}$.

\STATE \textbf{{Initialization}}: $\bm{h}^{0}=\bm{h}^{\star}$
and $\bm{x}^{0}=\bm{x}^{\star}$.

\STATE \textbf{{Gradient updates}}: \textbf{for }$t=0,1,\ldots,t_{0}-1$
\textbf{do}

\STATE \vspace{-1em}
 \begin{subequations}\label{subeq:gradient_update_ncvx-2} 
\begin{align}
\left[\begin{array}{c}
\boldsymbol{h}^{t+1/2}\\
\boldsymbol{x}^{t+1/2}
\end{array}\right]= & \left[\begin{array}{c}
\boldsymbol{h}^{t}\\
\boldsymbol{x}^{t}
\end{array}\right]-\eta\left[\begin{array}{c}
\nabla_{\boldsymbol{h}}f\left(\boldsymbol{h}^{t},\boldsymbol{x}^{t}\right)\\
\nabla_{\boldsymbol{x}}f\left(\boldsymbol{h}^{t},\boldsymbol{x}^{t}\right)
\end{array}\right],\\
\left[\begin{array}{c}
\boldsymbol{h}^{t+1}\\
\boldsymbol{x}^{t+1}
\end{array}\right]= & \left[\begin{array}{c}
\sqrt{\frac{\left\Vert \bm{x}^{t+1/2}\right\Vert _{2}}{\left\Vert \bm{h}^{t+1/2}\right\Vert _{2}}}\boldsymbol{h}^{t+1/2}\\
\sqrt{\frac{\left\Vert \bm{h}^{t+1/2}\right\Vert _{2}}{\left\Vert \bm{x}^{t+1/2}\right\Vert _{2}}}\boldsymbol{x}^{t+1/2}
\end{array}\right],
\end{align}
\end{subequations}where $\nabla_{\boldsymbol{h}}f(\cdot)$ and $\nabla_{\boldsymbol{x}}f(\cdot)$
represent the Wirtinger gradient (see \cite[Section 3.3]{li2019rapid}
and Appendix~\ref{subsec:Wirtinger-calculus}) of $f(\cdot)$ w.r.t.~$\bm{h}$
and $\bm{x}$, respectively.

\end{algorithmic}
\end{algorithm}

\paragraph{Properties of the auxiliary nonconvex algorithm.} The
trajectory of this auxiliary nonconvex algorithm enjoys several important
properties. In the following lemma, the results are stated for the
properly rescaled iterate
\[
\widetilde{\bm{z}}^{t}=\left(\widetilde{\bm{h}}^{t},\widetilde{\bm{x}}^{t}\right)\coloneqq\left(\frac{1}{\overline{\alpha^{t}}}\bm{h}^{t},\alpha^{t}\bm{x}^{t}\right),
\]
with alignment parameter defined by 
\[
\alpha^{t}\coloneqq\arg\min_{\alpha\in\mathbb{C}}\left\{ \left\Vert \frac{1}{\overline{\alpha}}\bm{h}^{t}-\bm{h}^{\star}\right\Vert _{2}^{2}+\left\Vert \alpha\bm{x}^{t}-\bm{x}^{\star}\right\Vert _{2}^{2}\right\} .
\]

\begin{lemma}\label{lemma:cvx-noncvx}Take $\lambda=C_{\lambda}\sigma\sqrt{K\log m}$
for some large enough constant $C_{\lambda}>0$. Assume the number
of measurements obeys $m\geq C\mu^{2}K\log^{9}m$ for some sufficiently
large constant $C>0$, and the noise satisfies $\sigma\sqrt{K\log m}\leq c/\log^{2}m$
for some sufficiently small constant $c>0$. Then, with probability
at least $1-O\left(m^{-100}+me^{-cK}\right)$ for some constant $c>0$,
the iterates $\left\{ \boldsymbol{h}^{t},\boldsymbol{x}^{t}\right\} _{0<t\leq t_{0}}$
of Algorithm (\ref{alg:gd-bd-ncvx-2}) satisfy \begin{subequations}\label{eq:intro-induction}
\begin{align}
\mathsf{dist}\left(\boldsymbol{z}^{t},\boldsymbol{z}^{\star}\right) & \leq\rho\mathsf{dist}\left(\boldsymbol{z}^{t-1},\boldsymbol{z}^{\star}\right)+C_{5}\eta\left(\lambda+\sigma\sqrt{K\log m}\right)\label{eq:induction1}\\
\max_{1\leq j\leq m}\left|\boldsymbol{a}_{j}^{\mathsf{H}}\big(\widetilde{\boldsymbol{x}}^{t}-\boldsymbol{x}^{\star}\big)\right| & \leq C_{7}\sqrt{\log m}\left(\lambda+\sigma\sqrt{K\log m}\right)\label{eq:induction3}\\
\max_{1\leq j\leq m}\left|\boldsymbol{b}_{j}^{\mathsf{H}}\widetilde{\boldsymbol{h}}^{t}\right| & \leq C_{8}\left(\frac{\mu}{\sqrt{m}}\log m+\sigma\right)\label{eq:induction4}\\
\max_{1\leq j\leq m}\left|\boldsymbol{b}_{j}^{\mathsf{H}}\big(\widetilde{\bm{h}}^{t}-\bm{h}^{\star}\big)\right| & \leq C_{9}\sigma\label{eq:incohc}
\end{align}
for any $0<t\leq t_{0}$, where $\rho=1-c_{\rho}\eta\in\left(0,1\right)$
for some small constant $c_{\rho}>0$, and we take $t_{0}=m^{20}$.
Here, $C_{5}$, $\ldots$, $C_{9}$ are constants obeying $C_{7}\gg C_{5}$.
In addition, we have 
\begin{equation}
\min_{0\leq t\leq t_{0}}\left\Vert \nabla f\left(\boldsymbol{h}^{t},\boldsymbol{x}^{t}\right)\right\Vert _{2}\leq\frac{\lambda}{m^{10}}.\label{eq:smallgradient}
\end{equation}
\end{subequations}\end{lemma}

Most of the inequalities of this lemma (as well as their proofs) resemble
the ones derived for Algorithm \ref{alg:gd-BD-ncvx} in Appendix \ref{appendix:noncvx}.
It is worth emphasizing, however, that the establishment of the inequality
(\ref{eq:incohc}) relies heavily on the idealized initialization
$(\bm{h}^{0},\bm{x}^{0})=(\bm{h}^{\star},\bm{x}^{\star})$, and the
current proof does not work if the algorithm is spectrally initialized.
The proof of this lemma is deferred to Appendix \ref{subsec:Proof-of-Lemmacvx-ncvx}. 

\paragraph{Connection between the approximate nonconvex minimizer and the convex solution.}

As it turns out, the above type of features of the nonconvex iterates
together with the first-order optimality of the convex program allows
us to control the proximity of the convex minimizer and the approximate
nonconvex optimizer. Before proceeding to develop this idea formally, we first introduce the following operators for notational convenience. For any $\bm{z}=[z_{j}]_{1\leq j\leq m}$ and any $\bm{Z}\in\mathbb{C}^{K\times K}$, we define
\begin{align}
\mathcal{A}\left(\bm{Z}\right) & \coloneqq\left\{ \bm{b}_{j}^{\mathsf{H}}\bm{Z}\bm{a}_{j}\right\} _{j=1}^{m},\qquad\mathcal{A}^{*}\left(\bm{z}\right)=\sum_{j=1}^{m}z_{j}\bm{b}_{j}\bm{a}_{j}^{\mathsf{H}},\nonumber \\
\mathcal{T}\left(\boldsymbol{Z}\right) & \coloneqq\mathcal{A}^{*}\mathcal{A}\left(\bm{Z}\right)=\sum_{j=1}^{m}\boldsymbol{b}_{j}\boldsymbol{b}_{j}^{\mathsf{H}}\bm{Z}\boldsymbol{a}_{j}\boldsymbol{a}_{j}^{\mathsf{H}}.\label{eq:operatordef}
\end{align}
Below are several key conditions on these operators concerned with the interplay between the noise size, the estimation
accuracy of the nonconvex estimate $(\bm{h}, \bm{x})$ and the regularization parameters $\lambda$. 

\begin{condition}\label{condition:fourier-lambda}
	The regularization parameter $\lambda$ satisfies
\begin{enumerate}
	\item $
	\| \mathcal{T}\left(\boldsymbol{h}\boldsymbol{x}^{\mathsf{H}}-\boldsymbol{h}^{\star}\boldsymbol{x}^{\star\mathsf{H}}\right)-\left(\boldsymbol{h}\boldsymbol{x}^{\mathsf{H}}-\boldsymbol{h}^{\star}\boldsymbol{x}^{\star\mathsf{H}}\right)\| <\lambda/8.
	$
	\item $
	\left\Vert \mathcal{A}^{*}\left(\bm{\xi}\right)\right\Vert =\|\sum_{j=1}^{m}\xi_{j}\boldsymbol{b}_{j}\boldsymbol{a}_{j}^{\mathsf{H}}\|\leq c\lambda,
	$ for some small constant $c>0$. 
\end{enumerate}
\end{condition}
Condition \ref{condition:fourier-lambda} requires that the regularization parameter $\lambda$ dominate the norm of the deviation of $\mathcal{T}(\boldsymbol{h}\boldsymbol{x}^{\mathsf{H}}-\boldsymbol{h}^{\star}\boldsymbol{x}^{\star\mathsf{H}})$ from its mean $\boldsymbol{h}\boldsymbol{x}^{\mathsf{H}}-\boldsymbol{h}^{\star}\boldsymbol{x}^{\star\mathsf{H}}$, and also the norm of the noise operated on by $\mathcal{A}^*$. As can be seen shortly, these two conditions can be met with high probability when $(\boldsymbol{h}, \boldsymbol{x})$ is sufficiently close to $(\boldsymbol{h}^{\star}, \boldsymbol{x}^{\star})$. 

Another critical condition is the following injectivity condition on $\mathcal{A}$. 
\begin{condition}\label{condition:fourier-inj}
	Let $T$ be the tangent space of $\boldsymbol{h}\boldsymbol{x}^{\mathsf{H}}$. Then for all $\boldsymbol{Z}\in T$, one has
	\[
	\left\Vert \mathcal{A}\left(\boldsymbol{Z}\right)\right\Vert _{2}^{2}\geq\frac{1}{16}\left\Vert \boldsymbol{Z}\right\Vert _{\mathrm{F}}^{2}.
	\]
\end{condition}

When these two conditions hold, the aforementioned intimate connection between approximate nonconvex minimizer and the convex solution can be formalized in the following crucial lemma. 

\begin{lemma}\label{lemma:proximity-convex-ncvx}
Suppose that $\left(\boldsymbol{h},\boldsymbol{x}\right)$ obeys\begin{subequations}\label{eq:hx-properties-all}
\begin{align}
\left\Vert \nabla f\left(\boldsymbol{h},\boldsymbol{x}\right)\right\Vert _{2}\leq C\frac{\lambda}{m^{10}},\label{eq:small-gradient}
\end{align}
\end{subequations}for some constants $C>0$. Then under Conditions \ref{condition:fourier-lambda} and \ref{condition:fourier-inj},
any minimizer $\boldsymbol{Z}_{\mathsf{cvx}}$ of the convex problem
(\ref{eq:objcvx}) satisfies
\[
\left\Vert \boldsymbol{h}\boldsymbol{x}^{\mathsf{H}}-\boldsymbol{Z}_{\mathsf{cvx}}\right\Vert _{\mathrm{F}}\lesssim\left\Vert \nabla f\left(\boldsymbol{h},\boldsymbol{x}\right)\right\Vert _{2}.
\]
\end{lemma}\begin{proof}See Appendix \ref{subsec:Proof-of-Lemma2}.\end{proof}
In words, if we can find a point $(\bm{h},\bm{x})$ that has vanishingly
small gradient (cf.~(\ref{eq:small-gradient})) and that satisfies the additional Conditions \ref{condition:fourier-lambda} and \ref{condition:fourier-inj}, 
then the matrix $\bm{h}\bm{x}^{\mathsf{H}}$ is guaranteed to be exceedingly
close to the solution of the convex program. Encouragingly, Lemma
\ref{lemma:cvx-noncvx} hints at the existence of a point along the
trajectory of Algorithm (\ref{alg:gd-bd-ncvx-2}) satisfying these
conditions (\ref{eq:hx-properties-all}); if this were true, then
one could transfer the properties of the approximate nonconvex optimizer
to the convex solution, as a means to certify the statistical efficiency
of convex programming. As we will see soon, this is indeed the case that with Assumption \ref{assumptions:models}, we can prove that under some mild sample size and noise level conditions, Conditions \ref{condition:fourier-lambda} and \ref{condition:fourier-inj} would hold with high probability. To begin with, the following lemma corresponds to the first point in Condition \ref{condition:fourier-lambda}.

\begin{lemma}\label{lemma:T-uniform-mean}Suppose that the sample
	complexity satisfies $m\geq C\mu^{2}K\log^{4}m$ for some sufficiently
	large constant $C>0$. Take $\lambda=C_{\lambda}\sigma\sqrt{K\log m}$
	for some large enough constant $C_{\lambda}>0$. Then with probability
	at least $1-O\left(m^{-10}+me^{-CK}\right)$, we have
	\[
	\left\Vert \mathcal{T}\left(\boldsymbol{h}\boldsymbol{x}^{\mathsf{H}}-\boldsymbol{h}^{\star}\boldsymbol{x}^{\star\mathsf{H}}\right)-\left(\boldsymbol{h}\boldsymbol{x}^{\mathsf{H}}-\boldsymbol{h}^{\star}\boldsymbol{x}^{\star\mathsf{H}}\right)\right\Vert <\lambda/8,
	\]
	simultaneously for any $\left(\boldsymbol{h},\boldsymbol{x}\right)$
	obeying \begin{subequations}\label{eq:hx-properties-all}
		\begin{align}
		\left\Vert \bm{h}\right\Vert _{2}=\left\Vert \bm{x}\right\Vert _{2},\quad\left\Vert \boldsymbol{h}-\boldsymbol{h}^{\star}\right\Vert _{2} & \leq\frac{C_{5}}{1-\rho}\eta\left(\lambda+\sigma\sqrt{K\log m}\right),\quad\left\Vert \boldsymbol{x}-\boldsymbol{x}^{\star}\right\Vert _{2}\leq\frac{C_{5}}{1-\rho}\eta\left(\lambda+\sigma\sqrt{K\log m}\right),\label{eq:hx-properties}\\
		\max_{1\leq j\leq m}\left|\boldsymbol{b}_{j}^{\mathsf{H}}\left(\bm{h}-\bm{h}^{\star}\right)\right| & \leq C_{9}\sigma\quad\text{and}\quad\max_{1\leq j\leq m}\left|\boldsymbol{a}_{j}^{\mathsf{H}}\left(\bm{x}-\boldsymbol{x}^{\star}\right)\right|\leq C_{7}\sqrt{\log m}\left(\lambda+\sigma\sqrt{K\log m}\right),\label{eq:hx-properties2}
		\end{align}
	\end{subequations}for some constants $C_{5},C_{7},C_{9}>0$. 
\end{lemma}\begin{proof}See Appendix \ref{subsec:Proof-of-Lemma8innoisy}.\end{proof}
Recall the definition of operator $\mathcal{T}$ in \eqref{eq:operatordef}.
The lemma above states that for all $(\bm{h},\bm{x})$ sufficiently
close to $(\bm{h}^{\star},\bm{x}^{\star})$, the matrix $\mathcal{T}\left(\boldsymbol{h}\boldsymbol{x}^{\mathsf{H}}-\boldsymbol{h}^{\star}\boldsymbol{x}^{\star\mathsf{H}}\right)$
is close to the expectation $\boldsymbol{h}\boldsymbol{x}^{\mathsf{H}}-\boldsymbol{h}^{\star}\boldsymbol{x}^{\star\mathsf{H}}$. 

Next we turn to the second point in Condition \ref{condition:fourier-lambda}. 
\begin{lemma}\label{lemma:noise}
	Suppose that Asumption \ref{assumptions:models} holds and $m\gtrsim K\log^{3}m$. With probability at least $1-O\left(m^{-100}\right)$,
	one has 
	\[
	\left\Vert \mathcal{A}^{*}\left(\bm{\xi}\right)\right\Vert =\Bigg\|\sum_{j=1}^{m}\xi_{j}\boldsymbol{b}_{j}\boldsymbol{a}_{j}^{\mathsf{H}}\Bigg\|\lesssim\sigma\sqrt{K\log m}.
	\]
\end{lemma}\begin{proof}See Appendix \ref{subsec:Proof-oflemmanoise}.\end{proof}

Regarding Condition \ref{condition:fourier-inj}, we have the following lemma.
\begin{lemma}\label{lemma:inj}Suppose that the sample complexity
	satisfies $m\geq C\mu^{2}K\log m$ for some sufficiently large constant
	$C>0$. Then with probability at least $1-O\left(m^{-10}\right)$,
	\[
	\left\Vert \mathcal{A}\left(\boldsymbol{Z}\right)\right\Vert _{2}^{2}\geq\frac{1}{16}\left\Vert \boldsymbol{Z}\right\Vert _{\mathrm{F}}^{2},\quad\forall\boldsymbol{Z}\in T
	\]
	holds simultaneously for all $T$ for which the associated point $\left(\boldsymbol{h},\boldsymbol{x}\right)$
	obeys \eqref{eq:hx-properties} and \eqref{eq:hx-properties2}. Here,
	$T$ denotes the tangent space of $\boldsymbol{h}\boldsymbol{x}^{\mathsf{H}}$.\end{lemma}\begin{proof}See
	Appendix \ref{subsec:Proof-of-Lemma-inj}.\end{proof}
Basically, this lemma
reveals that when $(\bm{h},\bm{x})$ is sufficiently close to $(\bm{h}^{\star},\bm{x}^{\star})$,
the operator $\mathcal{A}(\cdot)$ --- restricted to the tangent
space $T$ of $\bm{h}\bm{x}^{\mathsf{H}}$ --- is injective. 

%As we already proved previously in Lemma \ref{lemma:cvx-noncvx}, the auxiliary nonconvex algorithm might produce an approximate nonconvex optimizer satisfying \eqref{eq:hx-properties-all}, and hence admitting Conditions \ref{condition:fourier-lambda} and \ref{condition:fourier-inj} with high probability. 

Now we are ready to present the proof of Theorem \ref{theorem:cvx}.

\paragraph{Proof of Theorem \ref{theorem:cvx}.} Armed with this
result and the properties about the nonconvex trajectory, we are ready
to establish Theorem \ref{theorem:cvx} as follows. Let $\overline{t}\coloneqq\arg\min_{0\leq t\leq t_{0}}\left\Vert \nabla f\left(\boldsymbol{h}^{t},\boldsymbol{x}^{t}\right)\right\Vert _{\text{F}}$,
and take $\left(\boldsymbol{h}_{\mathsf{ncvx}},\boldsymbol{x}_{\mathsf{ncvx}}\right)=\left(\frac{1}{\overline{\alpha^{\overline{t}}}}\boldsymbol{h}^{\overline{t}},\alpha^{\overline{t}}\boldsymbol{x}^{\overline{t}}\right)$.
By virtue of Lemma \ref{lemma:cvx-noncvx}, we see that $\left(\boldsymbol{h}_{\mathsf{ncvx}},\boldsymbol{x}_{\mathsf{ncvx}}\right)$
satisfies --- with high probability --- the small gradient property
\eqref{eq:smallgradient} as well as all conditions required to invoke
Lemma \ref{lemma:proximity-convex-ncvx}. As a consequence, invoke
Lemma \ref{lemma:proximity-convex-ncvx} to obtain
\begin{equation}
\left\Vert \boldsymbol{Z}_{\mathsf{cvx}}-\boldsymbol{h}_{\mathsf{ncvx}}\boldsymbol{x}_{\mathsf{ncvx}}^{\mathsf{H}}\right\Vert _{\text{F}}\lesssim\frac{1}{c_{\text{inj}}}\left\Vert \nabla f\left(\boldsymbol{h}_{\mathsf{ncvx}},\boldsymbol{x}_{\mathsf{ncvx}}\right)\right\Vert _{\text{F}}\lesssim\text{\ensuremath{\frac{\lambda}{m^{10}}}}.\label{eq:proof-thm-cvx-1}
\end{equation}
Further, it is seen that
\begin{align}
\left\Vert \bm{h}_{\mathsf{ncvx}}\big(\bm{x}_{\mathsf{ncvx}}\big)^{\mathsf{H}}-\boldsymbol{h}^{\star}\boldsymbol{x}^{\mathsf{\star H}}\right\Vert _{\mathrm{F}} & \leq\left\Vert \bm{h}_{\mathsf{ncvx}}\big(\bm{x}_{\mathsf{ncvx}}\big)^{\mathsf{H}}-\bm{h}^{\star}\big(\bm{x}_{\mathsf{ncvx}}\big)^{\mathsf{H}}\right\Vert _{\mathrm{F}}+\left\Vert \bm{h}^{\star}\big(\bm{x}_{\mathsf{ncvx}}\big)^{\mathsf{H}}-\boldsymbol{h}^{\star}\boldsymbol{x}^{\mathsf{\star H}}\right\Vert _{\mathrm{F}}\nonumber \\
 & \leq\left\Vert \bm{h}_{\mathsf{ncvx}}-\bm{h}^{\star}\right\Vert _{2}\left\Vert \bm{x}_{\mathsf{ncvx}}\right\Vert _{2}+\left\Vert \bm{h}^{\star}\right\Vert _{2}\left\Vert \bm{x}_{\mathsf{ncvx}}-\boldsymbol{x}^{\mathsf{\star}}\right\Vert _{2}\nonumber \\
 & \leq2\left\Vert \bm{z}^{\star}\right\Vert _{2}\cdot\frac{C_{5}\eta}{\left(1-\rho\right)\left\Vert \bm{z}^{\star}\right\Vert _{2}}\left(\lambda+\sigma\sqrt{K\log m}\right)\nonumber \\
 & =\frac{2C_{5}}{c_{\rho}}\left(\lambda+\sigma\sqrt{K\log m}\right),\label{eq:proof-thm-cvx-2}
\end{align}
where the penultimate line follows from (\ref{eq:dist-bound-1}) and
the inequality
\[
\left\Vert \bm{x}_{\mathsf{ncvx}}\right\Vert _{2}\leq\left\Vert \bm{x}^{\star}\right\Vert _{2}+\left\Vert \bm{x}_{\mathsf{ncvx}}-\bm{x}^{\star}\right\Vert _{2}\leq\left\Vert \bm{z}^{\star}\right\Vert _{2}+\frac{C_{5}\eta}{\left(1-\rho\right)\left\Vert \bm{z}^{\star}\right\Vert _{2}}\left(\lambda+\sigma\sqrt{K\log m}\right)\leq2\left\Vert \bm{z}^{\star}\right\Vert _{2}.
\]
Taking (\ref{eq:proof-thm-cvx-1}) and (\ref{eq:proof-thm-cvx-2})
collectively yields
\begin{align*}
\left\Vert \boldsymbol{Z}_{\mathsf{cvx}}-\boldsymbol{h}^{\star}\boldsymbol{x}^{\mathsf{\star H}}\right\Vert _{\text{F}} & \leq\left\Vert \boldsymbol{Z}_{\mathsf{cvx}}-\boldsymbol{h}_{\mathsf{ncvx}}\boldsymbol{x}_{\mathsf{ncvx}}^{\mathsf{H}}\right\Vert _{\text{F}}+\left\Vert \boldsymbol{h}_{\mathsf{ncvx}}\boldsymbol{x}_{\mathsf{ncvx}}^{\mathsf{H}}-\boldsymbol{h}^{\star}\boldsymbol{x}^{\mathsf{\star H}}\right\Vert _{\text{F}}\\
 & \lesssim\frac{\lambda}{m^{10}}+\lambda+\sigma\sqrt{K\log m}\\
 & \lesssim\lambda+\sigma\sqrt{K\log m}.
\end{align*}
This together with the elementary bound $\left\Vert \boldsymbol{Z}_{\mathsf{cvx}}-\boldsymbol{h}^{\star}\boldsymbol{x}^{\mathsf{\star H}}\right\Vert \leq\left\Vert \boldsymbol{Z}_{\mathsf{cvx}}-\boldsymbol{h}^{\star}\boldsymbol{x}^{\mathsf{\star H}}\right\Vert _{\text{F}}$
concludes the proof, as long as the above key lemmas can be justified. 

To prove the results also holds for $\boldsymbol{Z}_{\mathsf{cvx,}1}$, we recall that $\boldsymbol{Z}_{\mathsf{cvx,}1}$ is the best rank-1 approximation of $\boldsymbol{Z}_{\mathsf{cvx}}$ and this implies that,
\[
\left\Vert \boldsymbol{Z}_{\mathsf{cvx}}-\boldsymbol{Z}_{\mathsf{cvx,}1}\right\Vert _{\text{F}} \leq \left\Vert \boldsymbol{Z}_{\mathsf{cvx}}-\boldsymbol{h}_{\mathsf{ncvx}}\boldsymbol{x}_{\mathsf{ncvx}}^{\mathsf{H}}\right\Vert _{\text{F}}\lesssim\text{\ensuremath{\frac{\lambda}{m^{10}}}}.
\]
Hence, repeating the above calculations for $\boldsymbol{Z}_{\mathsf{cvx,}1}$ reveals that \eqref{eq:thm:gaussian-cvx} continues to holds if $\boldsymbol{Z}_{\mathsf{cvx}}$ is replaced by $\boldsymbol{Z}_{\mathsf{cvx,}1}$.
